Distributed statistical inference with pyhf enabled through funcX

In High Energy Physics facilities that provide High Performance Computing environments provide an opportunity to efficiently perform the statistical inference required for analysis of data from the Large Hadron Collider, but can pose problems with orchestration and efficient scheduling. The compute architectures at these facilities do not easily support the Python compute model, and the configuration scheduling of batch jobs for physics often requires expertise in multiple job scheduling services. The combination of the pure-Python libraries pyhf and funcX reduces the common problem in HEP analyses of performing statistical inference with binned models, that would traditionally take multiple hours and bespoke scheduling, to an on-demand (fitting) "function as a service" that can scalably execute across workers in just a few minutes, offering reduced time to insight and inference. We demonstrate execution of a scalable workflow using funcX to simultaneously fit 125 signal hypotheses from a published ATLAS search for new physics using pyhf with a wall time of under 3 minutes. We additionally show performance comparisons for other physics analyses with openly published probability models and argue for a blueprint of fitting as a service systems at HPC centers.

==> Makefile <==
FILENAME = ms

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

LATEX = pdf 

BIBTEX = bibtex

default: document copy_draft

all: default

figures: $(figure_list)

figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

document: figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: deep_clean document
	
	sed -i.bak 's/cache=false/cache=true/' latex/packages.tex
	$(MAKE) document
	
	mkdir submit_to_arXiv
	cp CHEP_2021_proposal.tex submit_to_arXiv
	cp *.bbl submit_to_arXiv/ms.bbl
	cp -r src submit_to_arXiv
	cp -r latex submit_to_arXiv
	cp -r data submit_to_arXiv
	cp -r figures submit_to_arXiv
	cp Makefile submit_to_arXiv
	mv _minted-CHEP_2021_proposal submit_to_arXiv/_minted-ms
	mv submit_to_arXiv/CHEP_2021_proposal.tex submit_to_arXiv/ms.tex
	
	
	sed -i.bak '/^ *
	
	mv submit_to_arXiv/latex/webofc.cls submit_to_arXiv/webofc.cls
	sed -i.bak 's
	
	sed -i.bak '/{hyperref}/d' submit_to_arXiv/latex/packages.tex
	sed -i.bak '/hypersetup/d' submit_to_arXiv/latex/packages.tex
	
	
	sed -i.bak 's/finalizecache/frozencache/' submit_to_arXiv/latex/packages.tex
	
	find submit_to_arXiv/ -name "*.bak" -type f -delete
	
	find submit_to_arXiv/ -name "*.bib" -type f -delete
	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean
	if [ -f latex/packages.tex.bak ];then \
		mv latex/packages.tex.bak latex/packages.tex; \
	fi

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv


==> latex/packages.tex <==
\usepackage[varg]{txfonts}   % Web of Conferences font
\RequirePackage{caption}
\usepackage{amsmath,bm}
\graphicspath{{figures/}}
\usepackage{lineno}
\usepackage{booktabs}
\usepackage[normalem]{ulem}
\usepackage[cache=true,newfloat=true,frozencache]{minted}
\PassOptionsToPackage{hyphens}{url}
\usepackage[capitalize]{cleveref}% https://ctan.org/pkg/cleveref % Must be loaded after hyperref

\usemintedstyle{friendly}
\setminted[json]{fontsize=\scriptsize, numbersep=5pt, frame=lines, framesep=2mm, gobble=0}
\setminted[python]{fontsize=\scriptsize, numbersep=5pt, frame=lines, framesep=2mm, gobble=0, linenos}

% atlaspackage.sty

